Improving Code Review with GitHub Issue Tracking

Software quality is an important problem for technology companies, since it substantially impacts the efficiency, usefulness, and maintainability of the final product; hence, code review is a must-do activity for software developers. During the code review process, senior engineers monitor other developers' work to spot possible problems and enforce coding standards. One of the most widely used open-source software platforms, GitHub, attracts millions of developers who use it to store their projects. This study aims to analyze code quality on GitHub from the standpoint of code reviews. We examined the code review process using GitHub's Issues Tracker, which allows team members to evaluate, discuss, and share their opinions on the proposed code before it is approved. Based on our analysis, we present a novel approach for improving the code review process by promoting regularity and community involvement.

==> sections/future_works.tex <==
We only utilized a small number of GitHub repositories for this research. To achieve more precise findings, we would need to extend across a much larger data set, including repositories from other categories. Furthermore, we thought that popularity might reflect their expertise in our study into the relationship between experienced coders and good code quality. We want to discover a new way to analyze and measure a developer's skill in future projects. We would also like to work on monitoring the bugs discovered throughout the code review process to assess code quality.
